What Do LLMs Associate with Your Name? A Human-Centered Black-Box Audit of Personal Data

Large language models (LLMs), and conversational agents based on them, are exposed to personal data (PD) during pre-training and during user interactions. Prior work shows that PD can resurface, yet users lack insight into how strongly models associate specific information to their identity. We audit PD across eight LLMs (3 open-source; 5 API-based, including GPT-4o), introduce LMP2 (Language Model Privacy Probe), a human-centered, privacy-preserving audit tool refined through two formative studies (N=20), and run two studies with EU residents to capture (i) intuitions about LLM-generated PD (N1=155) and (ii) reactions to tool output (N2=303). We show empirically that models confidently generate multiple PD categories for well-known individuals. For everyday users, GPT-4o generates 11 features with 60% or more accuracy (e.g., gender, hair color, languages). Finally, 72% of participants sought control over model-generated associations with their name, raising questions about what counts as PD and whether data privacy rights should extend to LLMs.

==> chapters/legal_section.tex <==
\subsection{Conceptualizing Data Rights for LLMs: Legal Background}
\label{ssec:legal-llm-rights}

Across jurisdictions, regulators are debating how individual rights over personal data should extend to generative AI, such as LLMs. The European Union's General Data Protection Regulation (GDPR) provides one of the most influential frameworks, and thus serves as a useful reference point, even if not universally applicable. Under the GDPR, rights such as access, rectification, and erasure--the latter is often referred to by the public as ``right to be forgotten’’ (RTBF)--apply whenever \emph{personal data} are processed. Importantly, personal data is defined broadly: it includes not only information directly provided or indirectly collected, but also data that is inferred or generated if it relates to an identifiable person \cite{custers2024tell}. To make this more tangible, we distinguish between three categories\footnote{While the GDPR itself does not use this terminology, it provides a useful conceptual scaffold for analyzing LLM rights.}: \emph{direct data} (provided by the subject, see Art.\,13 GDPR), \emph{indirect data} (obtained from other sources, see Art.\,14 GDPR), and \emph{inferred data} (profiles or generated attributes, debated but recognized in legal scholarship \cite{custers_tell_2024,hauselmann2024right,rupp2024clarifying} and by EU regulators \cite{edpb2024opinion28}).

The right to erasure (Art.\,17 GDPR)--to generalize, we refer to it as RTBF throughout this paper--, illustrates the aforementioned challenge. It enables individuals to request deletion of their data when processing is unlawful, irrelevant, or consent is withdrawn. Search engines operationalized this via delisting \cite{Bertram2019FiveYearsRTBF,Vilella2025DeIndexingRTBF}, but LLMs store and reproduce information in fundamentally different ways. Memorized or inferred content is embedded in model parameters, making selective removal technically challenging, as we show below (\ref{ssec:tech-background}). As Zhang et al. (2024) note, unlike search indexes, LLMs blur boundaries between factual input, associative knowledge, and fabricated text, complicating the mapping between legal entitlements and technical fixes \cite{zhang2025right}. Figure~\ref{fig:rights-decision} visualizes a decision flow for when rights apply: First, whether an output is linked to an identifiable individual. Second, which type of data is at stake (direct, indirect, or inferred). Third, what remedies are feasible in practice. While the GDPR offers the clearest articulation, similar debates arise in other jurisdictions (e.g., California’s CPRA, India’s DPDP Act).% The broader issue is global: how should law adapt when AI systems not only process but actively generate personal data?

\begin{figure}[H]
\centering
\setlength{\fboxsep}{6pt}\fbox{%
\parbox{0.92\linewidth}{
\textbf{Decision flow for personal data rights in LLMs:}\\
1.~Is the output linked to an identifiable person? If no, rights do not apply. If yes, continue.\\
2.~What type of data? \\
\hspace{0.7em}-- \emph{Direct:} provided by the subject (GDPR Art.\,13).\\
\hspace{0.7em}-- \emph{Indirect:} obtained from other sources (GDPR Art.\,14).\\
\hspace{0.7em}-- \emph{Inferred:} profiles or generated attributes (recognized in scholarship \cite{custers_tell_2024}).\\
3.~How do rights attach? \\
\hspace{0.7em}-- Access of Data: full for direct/indirect; partial for inferred.\\
\hspace{0.7em}-- Rectification of Data: full for direct/indirect; limited for inferred.\\
\hspace{0.7em}-- Erasure of Data: applies to all, except abstract group profiles.\\
4.~Do exceptions apply (e.g., freedom of expression, public interest)?\\
5.~Which remedies are feasible?}}
\caption{Conditions under which personal data rights may apply to LLMs, illustrated using the GDPR as a case study. The categories of direct, indirect, and inferred data are a conceptual scaffold grounded in GDPR provisions (Arts.\,13–14) and legal scholarship.}
\label{fig:rights-decision}
\end{figure}

However, our conversations with EU Data Privacy lawyers highlight a broad deadlock in formalizing this decision flow. On the one hand, computer scientists and providers of LLMs seek legal clarity on when generated text should be treated as personal data. On the other, legal researchers, NGOs, and regulators demand empirical demonstrations of risk before making determinations. Yet the law's expectation of deterministic ``proof’’ is difficult to reconcile with the probabilistic nature of neural networks. This impasse underscores the need for interdisciplinary tools and human-centered studies that can translate abstract legal principles into actionable signals for both users and regulators. This motivates our turn to the technical background and related work, where we highlight the gaps this work aims to address.



